Physarum polycephalum: Smart network adaptation

Life evolved organisms to adapt dynamically to their environment and autonomously exhibit behaviours. While complex behaviours in organisms are typically associated with the capability of neurons to process information, the unicellular organism Physarum polycephalum disabuses us by solving complex tasks despite being just a single although gigantic cell shaped into a mesmerizing tubular network. In Physarum, smart behaviours arise as network tubes grow or shrink due to the mechanochemical coupling of contractile tubes, fluid flows and transport across the network. Here, from a physicist's perspective, we introduce the biology and active chemo-mechanics of this living matter network. We then review Physarum's global response in migration and dynamic state to its environment before revisiting its network architecture and flow and transport patterns. Finally, we summarize recent studies on storing and processing information to mount well-informed behaviours.

==> comment.tex <==
\begin{comment}
Thank you again for agreeing to write an article on The Development of the Slime Mold Physarum for Volume 14 of the Annual Review of Condensed Matter Physics. A brief summary of Annual Reviews guidelines regarding manuscript preparation and submission appears below.
 
DEADLINE: 
Your manuscript is due on April 1, 2022. If you will not be able to submit by this date, please get in touch as soon as possible. Because of the parameters of our production schedule, we cannot guarantee publication of overlength manuscripts or manuscripts received after this deadline. With regret, we are not able to grant extensions this year (even requests for only a week or two), so please plan to submit by the due date. If you know that you will not be able to meet this deadline, please let me know sooner than later. We do generally offer one-time deferrals to authors who cannot submit by this date, but we cannot guarantee whether it will be a one-year or two-year deferral (timing will depend on the number of deferral requests received).
 
LENGTH:
We ask that you limit the review to 8,400 words of main text and a maximum of 150 references—counts that will produce our desired 20 typeset pages. Please note that each small figure or table requires space approximately equal to 300 words of text and each large one 600 words; thus, for every figure/table, subtract the appropriate number of words from your total allotment. Be sure to include a brief abstract (150 words at maximum) as well as up to 6 keywords associated with your topic; do not include these elements in your word count.
 
Overlength manuscripts will be returned for length reduction, so please make every effort to adhere to the specified allotment. Our article length estimator, available at the following URL, can help you monitor length as you prepare your submission: http://www.annualreviews.org/page/authors/general-information. Access it by selecting the name of your journal from the drop-down list under Article Preparation and Submission. 
 
STYLE/FORMAT:
While preparing your submission, please consult the Instructions for the Preparation of Manuscripts and Annual Reviews Graphics Guide, available online at http://www.annualreviews.org/page/authors/general-information (select the name of your journal from the drop-down list under Article Preparation and Submission). It is important that you follow our house style in the manuscript preparation stage; otherwise, new errors might be introduced in later correction and revision.
 
HOW TO SUBMIT:
Please submit your manuscript via our online submission form (you do not need to log in or create an account to do so):
https://annualreviews.sharefile.com/r-r845a371cfed45ed9 
For easier uploading, we recommend that you put all of your files in one folder, compress the folder (using WinZip, StuffIt, or Gzip), and then upload the single compressed file.
Please review the first part of the What to Send section below before you upload your file to ensure that you submit a complete manuscript.
The website will display a confirmation message when your file has been successfully uploaded and will also send an email notification. (If you do not receive the latter in your inbox, please check your junk/spam folder.)
 
WHAT TO SEND:
Send us your final version only. Please provide complete contact information for all authors, especially email addresses. A detailed checklist describing all required and optional elements is available online at http://www.annualreviews.org/page/authors/general-information (select the name of your journal from the drop-down list under Article Preparation and Submission). 
We request that you submit:
 
an editable text file of the main text (LaTeX or Microsoft Word) and any tables (LaTeX, Microsoft Word, or Microsoft Excel);
editable graphics files (see Graphics Guide for preferred formats);
a PDF file of the entire manuscript, including all figures and tables; and
a separate PDF file containing the figures only.
 
As part of your manuscript, you may provide the following optional material:
 

Terms and Definitions list (as many as 20, at ≤20 words each)
Summary Points list (as many as 8, in complete sentences)
Future Issues list (as many as 8, in complete sentences)
Reference Annotations (as many as 10, at ≤15 words each)
Related Resources list (as many as 10)
Sidebar(s) (50–200 words each, called out in the main text)
 
References: Please follow the guidelines in the Instructions for the Preparation of Manuscripts for literature citations; Literature Cited sections that do not follow our house style will be sent back to you for reformatting. References in the Literature Cited section in the Annual Review of Condensed Matter Physics are numbered sequentially, in order of appearance. Note that all sources listed in Literature Cited must be cited within the text, and all sources cited within the text must be listed in Literature Cited.
 
If you are using EndNote, you can download the appropriate style from http://www.annualreviews.org/page/authors/author-instructions/preparing/endnotes. After you have downloaded the style, save it directly into your EndNote library, then reformat the manuscript with that style. This will ensure you are using the current version of the style (your EndNote program may have an outdated version).
 
Graphics: If your review includes figures, please refer to the Annual Reviews Graphics Guide (available online at http://www.annualreviews.org/page/authors/general-information; select the name of your journal from the drop-down list under Article Preparation and Submission). All figures must be mentioned in the main text. If you are using previously published figures, you are responsible for obtaining permission from the copyright holder and providing the correct credit line.
 
Enhanced Graphics (Optional): Annual Reviews welcomes the submission of author-created videos and animations. In addition, the Illustration Department can help with the creation of enhanced graphics, such as images with embedded hyperlinks.
 
Supplemental Material (Optional): In addition to enhanced graphics, lengthy tables and other extensive electronic materials can be posted as Supplemental Material on our website and hyperlinked to the online versions of your article. Our Supplemental Material policy is available at http://www.annualreviews.org/page/authors/author-instructions/preparing/supmat.
We sincerely thank you for the efforts that go into your contribution. If you have any questions, please get in touch.
\end{comment}
